The Paradox Of Just-in-Time Liquidity in Decentralized Exchanges: More Providers Can Sometimes Mean Less Liquidity

We study Just-in-time (JIT) liquidity provision in blockchain-based decentralized exchanges. A JIT liquidity provider (LP) monitors pending swap orders in public mempools of blockchains to sandwich orders of their choice with liquidity, depositing right before and withdrawing right after the order. Our game-theoretic model with asymmetrically informed agents reveals that a JIT LP's presence does not always enhance liquidity pool depth, as one might expect. While passive LPs face adverse selection by informed arbitrageurs, a JIT LP's ability to detect pending orders for toxic order flow prior to liquidity provision lets them avoid being adversely selected. JIT LPs thus only provide liquidity to uninformed orders and crowd out passive LPs when order volume is not sufficiently elastic to pool depth, possibly reducing overall market liquidity. We show that using a two-tiered fee structure which transfers a part of a JIT LP's fee revenue to passive LPs or allowing for JIT LPs to compete \`{a} la Cournot are potential solutions to mitigate the negative effects of JIT liquidity.

==> old/competition.tex <==
\section{Competing Just-in-Time Liquidity Providers}\label{sec:competition}

% \textcolor{blue}{intro; modeling assumptions}

In this extension of the model, we consider the case of two competing JIT LPs, indexed by $j\in\{1,2\}$. In practice, if multiple JIT LPs submit orders to sandwich a swap with liquidity, the validator picks only one of them to confirm in the block, typically via a gas fee auction. This reduces to our baseline model with an extra process to determine which JIT LP's transactions to confirm. We instead suppose that the JIT LPs compose \`{a} la Cournot by assuming that both JIT LPs' sandwich orders are confirmed. The description of Period 3 are thus modified as follows.

\paragraph{Period 3 (Competitive Setting): JIT LPs Decide Whether to Provide Liquidity} Each JIT LP is endowed with $e_J=\bar{\nu}e_P$ risky coins and $pe_J$ stable coins, and arrives independently of the other JIT LP in Period 3 with probability $\pi\in[0,1]$. In addition to knowing whether an informed or uninformed trader submitted the swap order, we also assume that each JIT LP has a monitoring technology that tells them whether their competitor has arrived or not. JIT LP $j$ submits an order to deposit $d_J^{(j)}$ risky coins and $pd_J^{(j)}$ stable coins immediately before the swap, and an order to withdraw its share of the pool immediately after the swap. Note that the specific ordering of the deposit orders does not affect the JIT LPs' payoffs as long as both are placed before the swap order. The same is true for the ordering of the withdrawal orders as long as both are placed after the swap order. We take Assumptions 1 and 2* to hold in this extension, and formalize the monitoring technology assumption in what follows.  \\[-0.75\baselineskip]

\noindent \textbf{\textsc{Assumption 2*.}}
\textit{We assume that for any $\zeta,\zeta_U\in[\underline{\zeta},\overline{\zeta}]$, conditional on a single JIT arriving, the JIT LP's liquidity constraint does not bind in any equilibrium (if at least one exists).} \\[-0.75\baselineskip]

\noindent \textbf{\textsc{Assumption 3.}}
\textit{Denote the set of arrival scenarios as $\Omega_1=\{\textsf{NA}_2,\textsf{A}_2\}$ and $\Omega_2=\{\textsf{NA}_1,\textsf{A}_1\}$, where $\textsf{NA}_{-j}$ corresponds to the event that JIT LP $j$'s competitor did not arrive and $\textsf{A}_{-j}$ corresponds to the event that JIT LP $j$'s competitor arrived. We assume that JIT LP $j$, for $j\in\{1,2\}$, can distinguish between  scenarios in $\Omega_j$ in making their deposit decision.} \\[-0.75\baselineskip]

The strategy space of JIT LP $j$ is now
\begin{align*}
    d_J^{(j)}:[0,e_P]\times([0,e_P]\times\Omega\to\R_+^2\backslash\R_{++}^2)\times\Omega\times\Omega_j\to[0,e_J].
\end{align*}
Under this assumption, conditional on the arrival of JIT LP $j$, if they are in arrival scenario $\textsf{NA}_{-j}$, then they know that they have monopoly power in the JIT liquidity market and behave as the JIT LP in the baseline model. If they are in arrival scenario $\textsf{A}_{-j}$, then they are competing with the other JIT LP as well as the passive LPs for a share of the pool while also determining the swap order's price impact. The main features of the equilibrium outcome in the monopolist JIT case are preserved in the competitive case, with a extra outcome for the scenario in which both JIT LPs arrive.

\begin{theorem}\label{thm:competition-eq}
Under competition between JIT LPs, a non-trivial subgame-perfect Nash equilibrium exists if and only if $\zeta_U>\underline{\zeta}_U(f,\pi)$ where
\begin{align*}
    \underline{\zeta}_U(f,\pi)=\frac{2(1+f)^3}{2+\pi f(3+f)}.
\end{align*}
Moreover, this equilibrium is unique. In the equilibrium outcome:
\begin{itemize}
    \item The amount of passive liquidity provided is $d_P^\star=e_P\cdot\mathbbm{1}\{\alpha \mathcal{C} + (1-\alpha)\cdot\mathcal{R}_C(\pi)\geq0\}$.
    \item The value of the informed trader's buy and sell swap orders is $\mu_Id_P^\star$ for some constant $\mu_I$ where $\mu_I$ is the same constant as in Theorem \ref{thm:passive-br}. 
    \item The value of the uninformed trader's buy and sell swap order is $\mu_C(\pi)\cdot d_P^\star$ for some function $\mu_C(\pi)$ that is increasing in $\pi$. Moreover, $\mu_C(\pi)\geq\mu(\pi)$ in Theorem \ref{thm:passive-br} for all $\pi\in[0,1]$.
    \item Conditional on the arrival of a single JIT LP, the arriving JIT LP, denoted by $j$, provides liquidity only when facing an uninformed trader. The amount of JIT liquidity provided by the arriving JIT LP is $d_J^{(j)\star}=\nu(\pi)\cdot d_P^\star$, where $\nu(\pi)$ is the same as in Theorem \ref{thm:passive-br}.
    \item Condition on the arrival of both JIT LPs, the arriving JIT LPs provide liquidity only when facing an uninformed trader. The amount of JIT liquidity provided by both JIT LPs $j\in\{1,2\}$ is $d_J^{(j)\star}=e_J$.
\end{itemize}
\end{theorem}

A crucial difference in this equilibrium, compare to that of the baseline model with a single JIT LP, is the behavior of JIT LPs conditional on both arriving. Each JIT LP has to vie for a share of the pool not only with the passive LPs, but also with their competitor. In the appendices, we show that as a lemma, a JIT LP's optimal deposit amount must give a share of the pool that is over one-half. Since the competing JIT LPs cannot both own more than half of the pool, they have an incentive to deposit more liquidity until their endowment is reached. 

Here, Assumption 2* plays a critical role. Since the optimal deposit amount when there is one JIT LP in the market is assumed to not exceed the JIT LP's endowment, the optimal deposit amount when both JIT LPs arrive exceeds that when only one arrives. For the uninformed trader, this means that expected additional liquidity in the competitive setting is greater than that in the monopolist setting, yielding a higher equilibrium uninformed trading volume under competition.

\begin{theorem}\label{thm:threshold-comp}
Let $\pi\in(0,1)$. Suppose that a unique equilibrium exists when the each JIT LP's  arrival probability is $\pi$ for all private value shock sizes $\zeta_U\in[\underline{\zeta},\overline{\zeta}]$, holding the other exogenous parameters fixed. Then one of the following is true:
\begin{itemize}
    \item The JIT LPs complement the passive LPs at arrival probability $\pi$ for all $\zeta_U\in[\underline{\zeta},\overline{\zeta}]$.
    \item The JIT LPs crowd out the passive LPs at arrival probability $\pi$ for all $\zeta_U\in[\underline{\zeta},\overline{\zeta}]$.
    \item There exists $\zeta^\star_C(f,\pi)\in[\underline{\zeta},\overline{\zeta}]$ such that the JIT LP complements the passive LPs at arrival probability $\pi$ if and only if $\zeta_U\geq\zeta^\star_C(f,\pi)$.
\end{itemize}
Moreover, $\zeta^\star_C(f,\pi)\leq\zeta^\star(f,\pi)$ for all $\pi\in(0,1)$ where $\zeta^\star(f,\pi)$ is the threshold described in Theorem \ref{thm:threshold} that corresponds to the setting of a single JIT LP.
\end{theorem}

In the competitive setting, there also exists a threshold $\zeta^\star_C(f,\pi)$ that delineates regimes of $\zeta_U$ where the competing JIT LPs crowd out the passive LPs ($\zeta^\star_C(f,\pi)$) and where the competing JIT LPs complement the JIT LPs ($\zeta^\star_C(f,\pi)$). Additionally, the threshold at which the JIT LP(s) switch from crowding out to complementing the passive LPs is lower under competition than under a monopolist JIT LP. Then holding all parameters fixed, there exist values of $\zeta_U$ where a single JIT LP crowds out passive LPs yet competing JIT LPs complement passive LPs, but not vice versa. This means that the uninformed trader's demand is much more sensitive relative to expected pool depth under competition, as less of an increase in $\zeta_U$ is needed to induce a proportionally higher trading volume relative to liquidity provided.



\paragraph{Robustness of the Two-Tiered Fee Structure Under Competition}

In the appendices, we show that the key features of the two-tiered fee structure from Section \ref{sec:ttfs} are preserved in the setting of competing JIT LPs. In equilibrium, the uninformed trader's swap size and JIT LP's deposit size conditional on the arrival of one JIT LP still decrease as more fee revenue is transferred away from the JIT LP. We derive thresholds $\bar{f}(\pi)$ and $\hat{\zeta}_C(f,\pi)$ such that $f\in[0,\bar{f}(\pi))$ and $\zeta_U\geq\hat{\zeta}_C(f,\pi)$ is a sufficient condition for the passive LPs' per-unit utility to decrease in $\lambda$ across the entire range of $\lambda$. Similarly, welfare increases in $\lambda$ as long as that the passive LPs do not drop out of the market; if so, then welfare is zero.

\section{Robustness of the Two-Tiered Fee Structure Under Competition}

We state the analogous versions of results \ref{thm:twotier-eq}--\ref{thm:maxwelfare} in the competitive setting.

\begin{theorem}\label{thm:competition-twotier-eq}
Under competition between JIT LPs and a two-tiered fee structure with transfer rate $\lambda\in[0,1]$, a non-trivial subgame-perfect Nash equilibrium exists if and only if $\zeta_U > \underline{\zeta}_U(f,\lambda,\pi)$, where
\begin{align*}
    \underline{\zeta}_U(f,\lambda,\pi) = \frac{2(1+f)^3}{2+\pi[(2+f)\sqrt{(1+f)(1+\lambda f)}-2]}.
\end{align*}
Moreover, this equilibrium is unique. In the equilibrium outcome:
\begin{itemize}
    \item The amount of passive liquidity provided
    is $d_P^\star=e_P\cdot\mathbbm{1}\{\alpha \mathcal{C} + (1-\alpha)\cdot\mathcal{R}_C(\lambda,\pi)\geq0\}$.
    \item The value of the informed trader's buy and sell swap orders is $\mu_Id_P^\star$ where $\mu_I$ is the same constant as in Theorem \ref{thm:passive-br}.
    \item The value of the uninformed trader's buy and sell swap orders is $\mu_C(\lambda,\pi)$ for some function $\mu_C(\lambda,\pi)$ that is increasing in $\pi$. Moreover, $\mu_C(\lambda,\pi)\geq\mu(\lambda,\pi)$ in Theorem \ref{thm:twotier-eq} for all $\pi\in[0,1]$ and $\lambda\in[0,1]$.
    \item Conditional on the arrival of a single JIT LP, the arriving JIT LP, denoted by $j$, provides liquidity only when facing an uninformed trader. The amount of JIT liquidity provided is $d_J^\star=\nu(\lambda,\pi)\cdot d_P^\star$, where $\nu(\lambda,\pi)$ is the same as in Theorem \ref{thm:twotier-eq}.
    \item Conditional on the arrival of both JIT LPs, the arriving JIT LPs provide liquidity only when facing an uninformed trader. The amount of JIT provided by both JIT LPs $j\in\{1,2\}$ is $d_J^{(j)\star}=e_J$.
\end{itemize}
\end{theorem}

\begin{proposition}\label{thm:competition-dampen}
Let $\pi\in(0,1]$. Suppose that a unique non-trivial subgame-perfect Nash equilibrium for all $\lambda \in [0,1]$, holding the other exogenous parameters fixed. When $\lambda$ decreases, i.e.\!\, a larger proportion of fees is transferred from the JIT LP to the passive LPs:
\begin{itemize}
\setlength\itemsep{0em}
    \item Conditional on the arrival of a single JIT LP, the ratio of the JIT LP's deposit size to the amount of passive liquidity provided decreases.
    \item Conditional on the arrival of both JIT LPs, the ratio of the JIT LP's deposit size to the amount of passive liquidity provided is constant.
    \item The ratio of the uninformed trader's swap value to the amount of passive liquidity provided decreases.
\end{itemize}
\end{proposition}

\begin{theorem}\label{thm:competition-preventfreeze}
Let $\pi\in[0,1]$. Suppose that a unique non-trivial subgame-perfect Nash equilibrium exists for all $\lambda\in$ $[0,1]$, holding the other exogenous parameters fixed. If $f\in[0,\pi)$, then there exists $\hat{\zeta}_C(f,\pi)$ such that if $\zeta_U\geq\hat{\zeta}_C(f,\pi)$, then the passive LPs' per-unit utility decreases in $\lambda$ for all $\lambda\in[0,1]$.
\end{theorem}

\begin{theorem}\label{thm:compeition-maxwelfare}
Let $\pi\in[0,1]$. Suppose that a unique non-trivial subgame-perfect Nash equilibrium exists for all $\lambda \in$ $ [0,1]$, holding the other exogenous parameters fixed. Define $\mathcal{U}_C(\pi,\lambda)=\alpha\mathcal{C}+(1-\alpha)\cdot\mathcal{R}_C(\pi,\lambda)$. Then varying $\lambda$ results in the following effects on welfare:
\begin{itemize}
\setlength\itemsep{0em}
    \item If $\mathcal{U}_C(\pi,\lambda) < 0$ for all $\lambda \in [0,1]$, then welfare is zero for all $\lambda\in[0,1]$, reflecting a consistent absence of passive LP participation and a consequent market breakdown.
    \item Otherwise, if there exists $\lambda\in[0,1]$ such that $\mathcal{U}_C(\pi,\lambda)\geq0$, then welfare is maximized at the largest value of $\lambda$ at which passive LPs participate in the market, i.e.\!\, $\lambda^\star=\max\{\lambda\in[0,1]:\mathcal{U}_C(\pi,\lambda)\geq0\}$.
\end{itemize}
\end{theorem}

